CheapNVS: Real-Time On-Device Narrow-Baseline Novel View Synthesis

Single-view novel view synthesis (NVS) is a notorious problem due to its ill-posed nature, and often requires large, computationally expensive approaches to produce tangible results. In this paper, we propose CheapNVS: a fully end-to-end approach for narrow baseline single-view NVS based on a novel, efficient multiple encoder/decoder design trained in a multi-stage fashion. CheapNVS first approximates the laborious 3D image warping with lightweight learnable modules that are conditioned on the camera pose embeddings of the target view, and then performs inpainting on the occluded regions in parallel to achieve significant performance gains. Once trained on a subset of Open Images dataset, CheapNVS outperforms the state-of-the-art despite being 10 times faster and consuming 6% less memory. Furthermore, CheapNVS runs comfortably in real-time on mobile devices, reaching over 30 FPS on a Samsung Tab 9+.

==> table_comparison_new.tex <==
\begin{table*}[!t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|clllll|clllll|ccc}
& \multicolumn{6}{c|}{Open Images}  & \multicolumn{6}{c|}{COCO} & \multicolumn{3}{c}{Performance} \\
& \multicolumn{3}{c}{Warping} & \multicolumn{3}{c|}{Inpainting} & \multicolumn{3}{c}{Warping} & \multicolumn{3}{c|}{Inpainting} & \multicolumn{2}{c}{Runtime} & Memory \\ \hline
Method & \multicolumn{1}{l}{LPIPS$\downarrow$} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & \multicolumn{1}{l}{LPIPS$\downarrow$} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & GPU (ms)$\downarrow$ & \multicolumn{1}{l|}{Mobile (ms)$\downarrow$} & \multicolumn{1}{c}{GB}$\downarrow$ \\ \hline
Ours                                                    & \multicolumn{1}{l}{0.163} & 25.92       & 0.851        & 0.079            & 29.59            & 0.896                      & \multicolumn{1}{l}{0.112} & 26.16        & 0.884        & 0.066 & 28.32    & 0.897   &     \multicolumn{1}{c}{26}    & \multicolumn{1}{c|}{33}            &   0.14                    \\ \hline
Ours                                                    & \multicolumn{1}{l}{0.159}    & 25.75           & 0.848           & 0.073               & 30.03            &  0.903                               & \multicolumn{1}{l}{0.098}    & 26.89           & 0.899           & 0.056         & 29.30 & 0.913          &    26      & \multicolumn{1}{c|}{33}          &       0.14               \\ \hline
\end{tabular}}
\vspace{1mm}
    \caption{Results on COCO and Open Images. Rows 2 and 3 are models trained on Open Images, whereas the others are trained on COCO. OpenImages and COCO columns indicate evaluation on Open Images and COCO test sets. AdaMPI \cite{han2022single} performs the conventional warping we use as ground-truth, so we do not report its warping results. $\ddagger$ is AdaMPI trained on Open Images by us.} 
    \label{tab:comparison}
    \vspace{-7mm}
\end{table*}


